Learning Probabilistic Systems from Tree Samples

We consider the problem of learning a non-deterministic probabilistic system consistent with a given finite set of positive and negative tree samples. Consistency is defined with respect to strong simulation conformance. We propose learning algorithms that use traditional and a new "stochastic" state-space partitioning, the latter resulting in the minimum number of states. We then use them to solve the problem of "active learning", that uses a knowledgeable teacher to generate samples as counterexamples to simulation equivalence queries. We show that the problem is undecidable in general, but that it becomes decidable under a suitable condition on the teacher which comes naturally from the way samples are generated from failed simulation checks. The latter problem is shown to be undecidable if we impose an additional condition on the learner to always conjecture a "minimum state" hypothesis. We therefore propose a semi-algorithm using stochastic partitions. Finally, we apply the proposed (semi-) algorithms to infer intermediate assumptions in an automated assume-guarantee verification framework for probabilistic systems.

==> cex.tex <==
\section{Counterexamples to Simulation Conformance}
\label{sec:cex}
{\bf Corina: move this to background and make it shorter}

A counterexample is an important diagnostic information when simulation
conformance fails to hold; counterexamples are used by the learner in the active learning problem
we are interested in (Section \ref{sec:}). Let $L_1$ and $L_2$ be two LPTSes. We characterized a counterexample to $L_1
\preorder L_2$ as a tree previously \cite{KPC_cav12} and we only discuss it briefly
here. We first discuss what counterexamples are via a simple language-theoretic
characterization.

\begin{definition}[Language of an LPTS]
Given an LPTS $L$, we define its language, denoted $\L(L)$, as the set
$\{L' | L' ~\text{is an LPTS and } L' \preorder L\}$.
\end{definition}

\begin{lemma}
\label{lem:preorder_language}
$L_1 \preorder L_2$ iff $\L(L_1) \subseteq \L(L_2)$.
\end{lemma}

\begin{IEEEproof}
Necessity follows trivially from the transitivity of $\preorder$ and sufficiency
follows from the reflexivity of $\preorder$ which implies $L_1 \in \L(L_1)$.
\end{IEEEproof}

Thus, a counterexample $C$ can be defined as follows.

\begin{definition}[Counterexample]
\label{def:cex}
A counterexample to $L_1 \preorder L_2$ is an LPTS $C$ such that $C \in \L(L_1)
\setminus \L(L_2)$, i.e. $C \preorder L_1$ but $C \not\preorder L_2$.
\end{definition}

Now, $L_1$ itself is a trivial choice for $C$ but it does not give any more useful
information than what we had before checking the conformance.
Moreover, it is preferable to have $C$
with a special and simpler structure rather than a general LPTS as it helps in a more
efficient counterexample analysis, wherever it is
used. When the LPTSes are restricted to LTSes, a {\em tree-shaped} LTS is known
to be sufficient as a counterexample \cite{Chaki_thesis05}. Based on a similar
intuition, we show that it is a tree-shaped LPTS in the general, probabilistic, case.

\begin{theorem}
\label{thm:tree_cex}
If $L_1 \not\preorder L_2$, there is a tree which serves as a counterexample.
\end{theorem}

\begin{IEEEproof}
We only give a brief sketch of a constructive proof here.
Counterexample generation is based on the coarsest strong simulation computation from Section
\ref{sec:prelims}. By induction on the size of the current relation
$R$, we show that there is a tree counterexample to $s_1 \preorder
s_2$ whenever $(s_1, s_2)$ is removed from $R$. We only consider the
inductive case here. The pair is removed because there is a transition
$s_1 \trans{a} \mu_1$ but for every $s_2 \trans{a} \mu$,
$\mu_1 \not\dpreorder_R \mu$ \ie there exists $S^\mu_1
\subseteq S_1$ such that $\mu_1(S^\mu_1) >
\mu(R(S^\mu_1))$. Such an $S^\mu_1$ can be found in polynomial time and
space.
%cubic time and linear space.
Now, no pair in $S^\mu_1 \times
(\supp{\mu} \setminus R(S^\mu_1))$ is in $R$. By induction
hypothesis, a counterexample tree exists for each such pair. A
counterexample to $s_1 \preorder s_2$ is built using $\mu_1$ and
all these other trees.
\end{IEEEproof}

\begin{figure}
\centering
\includegraphics[scale=1.8]{figures/cex_eg.eps}
\caption{$C_p$, for $p \in (0,\frac{1}{2}]$, is a counterexample to $L_1
\preorder L_2$.}
\label{fig:cex_eg}
\end{figure}

For an illustration, see Figure \ref{fig:cex_eg} where $C_p$, for $p \in
(0,\frac{1}{2}]$ is a counterexample to $A \preorder B$. We also showed that structures simpler than trees are not
sufficient as counterexamples, in general \cite{KPC_cav12}.

We observe that the obtained counterexample $C$ is essentially a finite {\em tree execution} of
$L_1$. That is, there is a total mapping $M : S_C \to S_1$ such that for every
transition $c \trans{a} \mu_c$ of $C$, there exists $M(c) \trans{a} \mu_1$ such that $M$ restricted
to $\supp{\mu_c}$ is an injection and for every $c' \in \supp{\mu_c}$,
$\mu_c(c') = \mu_1(M(c'))$. Note that $M$ is also a strong simulation. We call
such a mapping an {\em execution mapping from $C$ to $L_1$} in the rest of the paper. An execution mapping is shown
in brackets beside the states of $C_p$ for $p = \frac{1}{2}$ in Figure \ref{fig:cex_eg}.
While the algorithm described in the above proof always generates
counterexamples with an {\em execution mapping}, it is possible to have a tree
counterexample, as per Definition \ref{def:cex}, without such a mapping. For
example, $C_p$ in Figure \ref{fig:cex_eg} for $p \in (0,\frac{1}{2})$ is also a
counterexample with no such {\em execution mapping}.

{\bf Corina: We will use this constructive proof when imposing conditions on the teacher in the active learning framework described in Section 5}.


==> results.tex <==
\section{Results}
We might discuss the one example which works both for partitions and stochastic
partitions - or might skip this section altogether.

